Searching for Localized Black-Hole solutions in Brane-World models

In the context of this thesis, the question that is going to occupy us, is the existence of a 5-dimensional braneworld black hole solution that is localized close to the 3-brane and has the properties of a regular 4-dimensional one. For this purpose, the 4-dimensional part of the complete 5-dimensional spacetime is considered to be a generalized Vaidya metric, in the context of which, the mass parameter $m$ is allowed to vary with respect to time, while it is also allowed to have both $y$ and $r$ dependence. The dependence on the $r$-coordinate essentially means that our black hole solution can deviate from the conventional Schwarzschild solution. Additionally, the dependence on the $y$-coordinate leads to a non-trivial profile of the black hole along the extra dimension. In order to justify physically the existence of such general mass parameter, we consider the case of two scalar fields $\phi(v,r,y)$, $\chi(v,r,y)$ which interact with each other and they are also non-minimally coupled to gravity via a general coupling function $f(\phi,\chi)$. In all the cases that were investigated in the context of this particular scenario, the result for the existence of a viable 5-dimensional localized black hole solution was negative, a result that causes concern about the compatibility of brane-world models with basic predictions of General Theory of Relativity.

==> Chapters/Chapter_Field_Theory.tex <==

\par All $25$ energy-momentum tensor's components ($T^M{}_N$) have explicitly calculated in the previous pages. Subsequently, the non-zero components in their compact form are
\begin{empheq}[box=\mymath]{align}\label{loc.93}
T^0{}_1&=e^{-2A}[(\pa_1\phi)^2+(\pa_1\chi)^2+\pa_1^2f]\nonum\\ \nonum\\
T^1{}_0&=e^{-2A}\left[(\pa_0\phi)^2+(\pa_0\chi)^2+\pa_0^2f+\left(1-\frac{2m}{r}\right)(\pa_1\pa_0\phi+\pa_1\chi\pa_0\chi+\pa_1\pa_0f)\right.\nonum\\
&\hspace{5em}\left. +\pa_1\left(\frac{m}{r}\right)\pa_0f-\pa_0\left(\frac{m}{r}\right)\pa_1f+e^{2A}\pa_4\left(\frac{m}{r}\right)\pa_4f\right]\nonum\\ \nonum\\
T^4{}_0&=\pa_4\phi\pa_0\phi+\pa_4\chi\pa_0\chi+\pa_4\pa_0f-A'\pa_0f-\frac{\pa_4m}{r}\pa_1f\nonum\\ \nonum\\
T^0{}_4&=e^{-2A}(\pa_1\phi\pa_4\phi+\pa_1\chi\pa_4\chi+\pa_1\pa_4f-A'\pa_1f)\nonum\\ \nonum\\
T^4{}_1&=e^{2A}T^0{}_4\nonum\\ \nonum\\
T^1{}_4&=e^{-2A}T^4{}_0+\left(1-\frac{2m}{r}\right)T^0{}_4\nonum\\ \nonum\\
T^0{}_0&=e^{-2A}\left[\pa_1\phi\pa_0\phi+\pa_1\chi\pa_0\chi+\pa_1\pa_0f-\pa_1\left(\frac{m}{r}\right)\pa_1f\right]+A'\pa_4f+\lagr-\square f\\ \nonum\\
T^1{}_1&=T^0{}_0+\left(1-\frac{2m}{r}\right)T^0{}_1\nonum\\ \nonum\\
T^2{}_2&=\frac{e^{-2A}}{r}\left[\pa_0f+\left(1-\frac{2m}{r}\right)\pa_1f\right]+A'\pa_4f+\lagr-\square f\nonum\\ \nonum\\
T^3{}_3&=T^2{}_2\nonum\\ \nonum\\
T^4{}_4&=(\pa_4\phi)^2+(\pa_4\chi)^2+\pa^2_4f+\lagr-\square f\nonum\\ \nonum\\
\lagr&=-\frac{e^{-2A}}{2}\left\{2(\pa_1\phi\pa_0\phi+\pa_1\chi\pa_0\chi)+\left(1-\frac{2m}{r}\right)[(\pa_1\phi)^2+(\pa_1\chi)^2]\right\}\nonum\\
&\hspace{5em}-\frac{1}{2}[(\pa_4\phi)^2+(\pa_4\chi)^2]-V(\phi,\chi)\nonum\\ \nonum\\
\square f&=e^{-2A}\pa_0\pa_1f+\frac{e^{-2A}}{r^2}\pa_1\left[r^2\pa_0f+r^2\left(1-\frac{2m}{r}\right)\pa_1f\right]+e^{-4A}\pa_4\left(e^{4A}\pa_4f\right)\nonum
\end{empheq}\\

\par The same components in their extended form are depicted below.
\begin{empheq}[box=\mymath]{align}\label{loc.94}
T^0{}_1&=\scriptstyle{e^{-2A}[(1+\pa_\phi^2f)(\pa_1\phi)^2+(1+\pa_\chi^2f)(\pa_1\chi)^2+2\pa_\chi\pa_\phi f\pa_1\chi\pa_1\phi+\pa_\phi f\pa_1^2\phi+\pa_\chi f\pa_1^2\chi]}\nonum\\ \nonum\\
T^1{}_0&=\scriptstyle{e^{-2A}}\left\{\scriptstyle{(1+\pa_\phi^2f)(\pa_0\phi)^2+(1+\pa_\chi^2f)(\pa_0\chi)^2+2\pa_\chi\pa_\phi f\pa_0\phi\pa_0\chi+\pa_\phi f\pa_0^2\phi+\pa_\chi f\pa_0^2\chi} \right.\nonum\\
&\hspace{2.7em}\scriptstyle{+\left(1-\frac{2m}{r}\right)[(1+\pa_\phi^2f)\pa_1\phi\pa_0\phi+(1+\pa_\chi^2f)\pa_1\chi\pa_0\chi+\pa_\phi\pa_\chi f(\pa_1\phi\pa_0\chi+\pa_1\chi\pa_0\phi)+\pa_\phi f\pa_1\pa_0\phi+\pa_\chi f\pa_1\pa_0\chi]}\nonum\\
&\hspace{2.7em}\left. \scriptstyle{+\left(\frac{\pa_1m}{r}-\frac{m}{r^2}\right)(\pa_\phi f\pa_0\phi+\pa_\chi f\pa_0\chi)-\frac{\pa_0m}{r}(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)+e^{2A}\frac{\pa_4m}{r}(\pa_\phi f\pa_4\phi+\pa_\chi f\pa_4\chi)}\right\}\nonum\\ \nonum\\
T^4{}_0&=(1+\pa_\phi^2f)\pa_4\phi\pa_0\phi+(1+\pa_\chi^2f)\pa_4\chi\pa_0\chi+\pa_\chi\pa_\phi f(\pa_4\chi\pa_0\phi+\pa_4\phi\pa_0\chi)\nonum\\
&\hspace{8.3em}+\pa_\phi f\pa_4\pa_0\phi+\pa_\chi f\pa_4\pa_0\chi-A'\pa_0f-\frac{\pa_4m}{r}\pa_1f\nonum\\ \nonum\\
T^0{}_4&=e^{-2A}[(1+\pa_\phi^2f)\pa_1\phi\pa_4\phi+(1+\pa_\chi^2f)\pa_1\chi\pa_4\chi+\pa_\phi\pa_\chi f(\pa_1\chi\pa_4\phi+\pa_1\phi\pa_4\chi) \nonum\\
&\hspace{10.2em}+\pa_\phi f\pa_1\pa_4\phi+\pa_\chi f\pa_1\pa_4\chi-A'(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)]\nonum\\ \nonum\\
T^4{}_1&=e^{2A}T^0{}_4\nonum\\ \nonum\\
T^1{}_4&=e^{-2A}T^4{}_0+\left(1-\frac{2m}{r}\right)T^0{}_4\\ \nonum\\
T^0{}_0&=e^{-2A}\left[\scriptstyle{(1+\pa_\phi^2f)\pa_1\phi\pa_0\phi+(1+\pa_\chi^2f)\pa_1\chi\pa_0\chi+\pa_\chi\pa_\phi f(\pa_1\chi\pa_0\phi+\pa_1\phi\pa_0\chi)+\pa_\phi f\pa_1\pa_0\phi}\right. \nonum\\
&\hspace{4.1em}\scriptstyle{+}\left.\scriptstyle{\pa_\chi f\pa_1\pa_0\chi+\frac{\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi}{r}\left(\frac{m}{r}-\pa_1m\right)}\right]\scriptstyle{+A'(\pa_\phi f\pa_4\phi+\pa_\chi f\pa_4\chi)+\lagr-\square f}\nonum\\ \nonum\\
T^1{}_1&=T^0{}_0+\left(1-\frac{2m}{r}\right)T^0{}_1\nonum\\ \nonum\\
T^2{}_2&=\frac{e^{-2A}}{r}\left[(\pa_\phi f\pa_0\phi+\pa_\chi f\pa_0\chi)+\left(1-\frac{2m}{r}\right)(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)\right]\nonum\\
&\hspace{4em}+A'(\pa_\phi f\pa_4\phi+\pa_\chi f\pa_4\chi)+\lagr-\square f\nonum\\ \nonum\\
T^3{}_3&=T^2{}_2\nonum\\ \nonum\\
T^4{}_4&=(1+\pa_\phi^2f)(\pa_4\phi)^2+(1+\pa_\chi^2f)(\pa_4\chi)^2+2\pa_\chi\pa_\phi f\pa_4\chi\pa_4\phi\nonum\\
&\hspace{8em}+\pa_\phi f\pa_4^2\phi+\pa_\chi f\pa_4^2\chi+\lagr-\square f\nonum\\ \nonum\\
\lagr&=-\frac{e^{-2A}}{2}\left\{2(\pa_1\phi\pa_0\phi+\pa_1\chi\pa_0\chi)+\left(1-\frac{2m}{r}\right)[(\pa_1\phi)^2+(\pa_1\chi)^2]\right\}\nonum\\
&\hspace{5em}-\frac{1}{2}[(\pa_4\phi)^2+(\pa_4\chi)^2]-V(\phi,\chi)\nonum\\ \nonum\\
\square f&=e^{-2A}\pa_0\pa_1f+\frac{e^{-2A}}{r^2}\pa_1\left[r^2\pa_0f+r^2\left(1-\frac{2m}{r}\right)\pa_1f\right]+e^{-4A}\pa_4\left(e^{4A}\pa_4f\right)\nonum
\end{empheq}

\newpage
\section{The Field Equations of the Theory}
\par Having in our disposal both Einstein tensor's components from equation \eqref{loc.7} and energy-momentum tensor's components from equation \eqref{loc.93} or \eqref{loc.94}, the independent field equations can immediately ensue with the use of equation \eqref{loc.14}. It is crystal clear that the independent field equations are the following.
\begin{center}
\underline{\large{Equation $(^0{}_1)$:}}\\
\end{center}
$$\eqref{loc.14}\xRightarrow[\eqref{loc.93}]{\eqref{loc.7}}f \underbrace{G^0{}_1}_{0}=T^0{}_1\Ra 0=e^{-2A}[(\pa_1\phi)^2+(\pa_1\chi)^2+\pa_1^2f]\Ra$$
\eq$\label{loc.95}
\boxed{(\pa_1\phi)^2+(\pa_1\chi)^2+\pa_1^2f=0}$
\par Substituting $\pa_1^2f$ from equation \eqref{loc.18} into \eqref{loc.95} we get\\
\eq$\label{loc.96}
\boxed{(1+\pa_\phi^2f)(\pa_1\phi)^2+(1+\pa_\chi^2f)(\pa_1\chi)^2+2\pa_\chi\pa_\phi f\pa_1\chi\pa_1\phi+\pa_\phi f\pa_1^2\phi+\pa_\chi f\pa_1^2\chi=0}$\\
\begin{center}
\underline{\large{Equation $(^1{}_0)$:}}\\
\end{center}
$$\eqref{loc.14}\xRightarrow[\eqref{loc.93}]{\eqref{loc.7}}T^1{}_0=f\ G^1{}_0\Ra$$
\begin{align}\label{loc.97}
&\scriptstyle{e^{-2A}}\left[\scriptstyle{(\pa_0\phi)^2+(\pa_0\chi)^2+\pa_0^2f+\left(1-\frac{2m}{r}\right)(\pa_1\pa_0\phi+\pa_1\chi\pa_0\chi+\pa_1\pa_0f)+\pa_1\left(\frac{m}{r}\right)\pa_0f-\pa_0\left(\frac{m}{r}\right)\pa_1f+e^{2A}\pa_4\left(\frac{m}{r}\right)\pa_4f}\right]\scriptstyle{=-f\frac{4 r A' \pa_4m+r \pa_4^2m-2 e^{-2 A} \pa_0m}{r^2}}\Ra\nonum\\ \nonum\\
&\boxed{\scriptstyle{(\pa_0\phi)^2+(\pa_0\chi)^2+\pa_0^2f+\left(1-\frac{2m}{r}\right)(\pa_1\phi\pa_0\phi+\pa_1\chi\pa_0\chi+\pa_1\pa_0f)+\pa_1\left(\frac{m}{r}\right)\pa_0f-\pa_0\left(\frac{m}{r}\right)\pa_1f+e^{2A}\pa_4\left(\frac{m}{r}\right)\pa_4f=f\left[\frac{2}{r^2}\pa_0m-\frac{e^{2A}}{r}(\pa_4^2m+4A'\pa_4m)\right]}}
\end{align}
\par The substitution of quantities $\pa_0^2f$ and $\pa_1\pa_0f$ from equations \eqref{loc.24} and \eqref{loc.25} respectively into equation \eqref{loc.97} yields to
\eq$\label{loc.98}
\boxed{\begin{array}{l}
\scriptstyle{e^{-2A}}\left\{\scriptstyle{(1+\pa_\phi^2f)(\pa_0\phi)^2+(1+\pa_\chi^2f)(\pa_0\chi)^2+2\pa_\chi\pa_\phi f\pa_0\phi\pa_0\chi+\pa_\phi f\pa_0^2\phi+\pa_\chi f\pa_0^2\chi} \right.\\
\hspace{2em}\scriptstyle{+\left(1-\frac{2m}{r}\right)[(1+\pa_\phi^2f)\pa_1\phi\pa_0\phi+(1+\pa_\chi^2f)\pa_1\chi\pa_0\chi+\pa_\phi\pa_\chi f(\pa_1\phi\pa_0\chi+\pa_1\chi\pa_0\phi)+\pa_\phi f\pa_1\pa_0\phi+\pa_\chi f\pa_1\pa_0\chi]}\\
\hspace{1.9em}\left.\scriptstyle{+\left(\frac{\pa_1m}{r}-\frac{m}{r^2}\right)(\pa_\phi f\pa_0\phi+\pa_\chi f\pa_0\chi)-\frac{\pa_0m}{r}(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)+e^{2A}\frac{\pa_4m}{r}(\pa_\phi f\pa_4\phi+\pa_\chi f\pa_4\chi)}\right\}\scriptstyle{=f\left[\frac{2}{r^2}\pa_0m-\frac{e^{2A}}{r}(\pa_4^2m+4A'\pa_4m)\right]}
\end{array}}$\\
\begin{center}
\underline{\large{Equation $(^4{}_0)$:}}\\
\end{center}
$$\eqref{loc.14}\xRightarrow[\eqref{loc.93}]{\eqref{loc.7}}T^4{}_0=f\ G^4{}_0\Ra\pa_4\phi\pa_0\phi+\pa_4\chi\pa_0\chi+\pa_4\pa_0f-A'\pa_0f-\frac{\pa_4m}{r}\pa_1f=f\frac{\pa_4m+r \pa_1\pa_4m}{r^2}\Ra$$
\eq$\label{loc.99}
\boxed{\pa_4\phi\pa_0\phi+\pa_4\chi\pa_0\chi+\pa_4\pa_0f-A'\pa_0f-\frac{\pa_4m}{r}\pa_1f=\frac{f}{r}\left(\frac{\pa_4m}{r}+\pa_1\pa_4m\right)}$

\newpage
The last equation in its extended form is:
\eq$\label{loc.100}
\boxed{\scriptstyle{(1+\pa_\phi^2f)\pa_4\phi\pa_0\phi+(1+\pa_\chi^2f)\pa_4\chi\pa_0\chi+\pa_\chi\pa_\phi f(\pa_4\chi\pa_0\phi+\pa_4\phi\pa_0\chi)+\pa_\phi f\pa_4\pa_0\phi+\pa_\chi f\pa_4\pa_0\chi-A'\pa_0f-\frac{\pa_4m}{r}(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)=\frac{f}{r}\left(\frac{\pa_4m}{r}+\pa_1\pa_4m\right)}}$\\
\begin{center}
\underline{\large{Equation $(^0{}_4)$:}}\\
\end{center}
$$\eqref{loc.14}\xRightarrow[\eqref{loc.93}]{\eqref{loc.7}}T^0{}_4=f\ \underbrace{G^0{}_4}_{0}\Ra e^{-2A}(\pa_1\phi\pa_4\phi+\pa_1\chi\pa_4\chi+\pa_1\pa_4f-A'\pa_1f)=0\Ra$$
\eq$\label{loc.101}
\boxed{\pa_1\phi\pa_4\phi+\pa_1\chi\pa_4\chi+\pa_1\pa_4f-A'\pa_1f=0}$\\
\par Using equation \eqref{loc.35} into equation \eqref{loc.101} we obtain
\eq$\label{loc.102}
\boxed{\scriptstyle{(1+\pa_\phi^2f)\pa_1\phi\pa_4\phi+(1+\pa_\chi^2f)\pa_1\chi\pa_4\chi+\pa_\phi\pa_\chi f(\pa_1\chi\pa_4\phi+\pa_1\phi\pa_4\chi)+\pa_\phi f\pa_1\pa_4\phi+\pa_\chi f\pa_1\pa_4\chi-A'(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)=0}}$\\
\begin{center}
\underline{\large{Equation $(^0{}_0)$:}}\\
\end{center}
$$\eqref{loc.14}\xRightarrow[\eqref{loc.93}]{\eqref{loc.7}}T^0{}_0-\Lambda_B=f\ G^0{}_0\Ra$$
\eq$\label{loc.103}
\boxed{\scriptstyle{e^{-2A}\left[\pa_1\phi\pa_0\phi+\pa_1\chi\pa_0\chi+\pa_1\pa_0f-\pa_1\left(\frac{m}{r}\right)\pa_1f\right]+A'\pa_4f+\lagr-\square f-\Lambda_B=f\left(6A'^2+3A''-\frac{2e^{-2A}}{r^2}\pa_1m\right)}}$\\
\par Equation \eqref{loc.103} is equivalent to
\eq$\label{loc.104}
\boxed{\begin{array}{l}
\scriptstyle{e^{-2A}}\left[\scriptstyle{(1+\pa_\phi^2f)\pa_1\phi\pa_0\phi+(1+\pa_\chi^2f)\pa_1\chi\pa_0\chi+\pa_\chi\pa_\phi f(\pa_1\chi\pa_0\phi+\pa_1\phi\pa_0\chi)+\pa_\phi f\pa_1\pa_0\phi+\pa_\chi f\pa_1\pa_0\chi+\frac{\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi}{r}\left(\frac{m}{r}-\pa_1m\right)}\right]\\
\hspace{3em}\scriptstyle{+A'(\pa_\phi f\pa_4\phi+\pa_\chi f\pa_4\chi)+\lagr-\square f-\Lambda_B=f\left(6A'^2+3A''-\frac{2e^{-2A}}{r^2}\pa_1m\right)}
\end{array}}$\\
\begin{center}
\underline{\large{Equation $(^2{}_2)$:}}\\
\end{center}
$$\eqref{loc.14}\xRightarrow[\eqref{loc.93}]{\eqref{loc.7}}T^2{}_2-\Lambda_B=f\ G^2{}_2\Ra$$
\eq$\label{loc.105}
\boxed{\frac{e^{-2A}}{r}\left[\pa_0f+\left(1-\frac{2m}{r}\right)\pa_1f\right]+A'\pa_4f+\lagr-\square f-\Lambda_B=f\left(6A'^2+3A''-\frac{e^{-2A}}{r}\pa_1^2m\right)}$\\
\par Expanding the partial derivatives of the function $f=f(\phi,\chi)$ we get
\eq$\label{loc.106}
\boxed{\scriptstyle{\frac{e^{-2A}}{r}\left[(\pa_\phi f\pa_0\phi+\pa_\chi f\pa_0\chi)+\left(1-\frac{2m}{r}\right)(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)\right]+A'(\pa_\phi f\pa_4\phi+\pa_\chi f\pa_4\chi)+\lagr-\square f-\Lambda_B=f\left(6A'^2+3A''-\frac{e^{-2A}}{r}\pa_1^2m\right)}}$

\newpage
\begin{center}
\underline{\large{Equation $(^4{}_4)$:}}\\
\end{center}
$$\eqref{loc.14}\xRightarrow[\eqref{loc.93}]{\eqref{loc.7}}T^4{}_4-\Lambda_B=f\ G^4{}_4\Ra$$
\eq$\label{loc.107}
\boxed{(\pa_4\phi)^2+(\pa_4\chi)^2+\pa^2_4f+\lagr-\square f-\Lambda_B=f\left(6A'^2-\frac{e^{-2A}}{r}\pa_1^2m-\frac{2e^{-2A}}{r^2}\pa_1m\right)}$\\
The combination of equations \eqref{loc.63} and \eqref{loc.107} gives
\eq$\label{loc.108}
\boxed{\scriptstyle{(1+\pa_\phi^2f)(\pa_4\phi)^2+(1+\pa_\chi^2f)(\pa_4\chi)^2+2\pa_\chi\pa_\phi f\pa_4\chi\pa_4\phi+\pa_\phi f\pa_4^2\phi+\pa_\chi f\pa_4^2\chi+\lagr-\square f-\Lambda_B=f\left(6A'^2-\frac{e^{-2A}}{r}\pa_1^2m-\frac{2e^{-2A}}{r^2}\pa_1m\right)}}$\\
\par Instead of using equations \eqref{loc.103}, \eqref{loc.105}, \eqref{loc.107} and the corresponding extended equations \eqref{loc.104}, \eqref{loc.106} and \eqref{loc.108}, which contain the terms $\lagr$ and $\square f$ that add extra complexity, we can be exempted from these terms by combining the aforementioned equations with each other.\\
\begin{center}
\underline{\large{Equation $(^0{}_0)-$Equation $(^2{}_2)$:}}\\
\end{center}
\par Subtracting equation \eqref{loc.105} from \eqref{loc.103} we get:\\
\eq$\label{loc.109}
\boxed{r(\pa_1\phi\pa_0\phi+\pa_1\chi\pa_0\chi+\pa_1\pa_0f)-\pa_0f-\pa_1f\left(\pa_1m+1-\frac{3m}{r}\right)=f\left(\pa_1^2m-\frac{2}{r}\pa_1m\right)}$\\
\par Correspondingly, from equations \eqref{loc.106} and \eqref{loc.104} one obtains
\eq$\label{loc.110}
\boxed{\begin{gathered}
r[(1+\pa_\phi^2f)\pa_1\phi\pa_0\phi+(1+\pa_\chi^2f)\pa_1\chi\pa_0\chi+\pa_\phi\pa_\chi f(\pa_1\chi\pa_0\phi+\pa_1\phi\pa_0\chi)+\pa_\phi f\pa_1\pa_0\phi+\pa_\chi f\pa_1\pa_0\chi] \\
-(\pa_\phi f\pa_0\phi+\pa_\chi f\pa_0\chi)-\left(\pa_1m+1-\frac{3m}{r}\right)(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)=f\left(\pa_1^2m-\frac{2}{r}\pa_1m\right)
\end{gathered}}$\\
\begin{center}
\underline{\large{Equation $(^0{}_0)-$Equation $(^4{}_4)$:}}\\
\end{center}
\par In the same way, subtracting equation \eqref{loc.107} from \eqref{loc.103} and \eqref{loc.108} from \eqref{loc.104} we respectively have:
\eq$\label{loc.111}
\boxed{\scriptstyle{e^{-2A}\left[\pa_1\phi\pa_0\phi+\pa_1\chi\pa_0\chi+\pa_1\pa_0f-\pa_1\left(\frac{m}{r}\right)\pa_1f\right]+A'\pa_4f-(\pa_4\phi)^2-(\pa_4\chi)^2-\pa_4^2f=f\left(3A''+\frac{e^{-2A}}{r}\pa_1^2m\right)}}$
\eq$\label{loc.112}
\boxed{\begin{gathered}
\scriptstyle{e^{-2A}\left[(1+\pa_\phi^2f)\pa_1\phi\pa_0\phi+(1+\pa_\chi^2f)\pa_1\chi\pa_0\chi+\pa_\phi\pa_\chi f(\pa_1\chi\pa_0\phi+\pa_1\phi\pa_0\chi)+\pa_\phi f\pa_1\pa_0\phi+\pa_\chi f\pa_1\pa_0\chi-\pa_1\left(\frac{m}{r}\right)(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)\right]}\\
\scriptstyle{+A'(\pa_\phi f\pa_4\phi+\pa_\chi f\pa_4\chi)-(1+\pa_\phi^2f)(\pa_4\phi)^2-(1+\pa_\chi^2f)(\pa_4\chi)^2-2\pa_\phi\pa_\chi f\pa_4\phi\pa_4\chi-\pa_\phi f\pa_4^2\phi-\pa_\chi f\pa_4^2\chi=f\left(3A''+\frac{e^{-2A}}{r}\pa_1^2m\right)}
\end{gathered}}$
\newpage
\begin{center}
\underline{\large{Equation $(^2{}_2)-$Equation $(^4{}_4)$:}}\\
\end{center}
\par Finally, the last field equation that has no dependence on the quantities $\lagr$ and $\square f$ can be provided by equations \eqref{loc.105} and \eqref{loc.107} or equations \eqref{loc.106} and \eqref{loc.108}. We respectively obtain
\eq$\label{loc.113}
\boxed{\frac{e^{-2A}}{r}\left[\pa_0f+\left(1-\frac{2m}{r}\right)\pa_1f\right]+A'\pa_4f-(\pa_4\phi)^2-(\pa_4\chi)^2-\pa_4^2f=f\left(3A''+\frac{2e^{-2A}}{r^2}\pa_1m\right)}$\\
\eq$\label{loc.114}
\boxed{\begin{gathered}
\frac{e^{-2A}}{r}\left[\pa_\phi f\pa_0\phi+\pa_\chi f\pa_0\chi+\left(1-\frac{2m}{r}\right)(\pa_\phi f\pa_1\phi+\pa_\chi f\pa_1\chi)\right]+A'(\pa_\phi f\pa_4\phi+\pa_\chi f\pa_4\chi)\\
-(1+\pa_\phi^2f)(\pa_4\phi)^2-(1+\pa_\chi^2f)(\pa_4\chi)^2-2\pa_\phi\pa_\chi f\pa_4\phi\pa_4\chi-\pa_\phi f\pa_4^2\phi-\pa_\chi f\pa_4^2\chi=f\left(3A''+\frac{e^{-2A}}{r}\pa_1^2m\right)\end{gathered}}$\\
\par Subsequently, we sum up the field equations that will be used in the next section, in an attempt to solve them and determine an acceptable mass function $m(v,r,y)$ that could localize the 5-D black hole on our 4-D universe. The field equations in their compact form are given by equations \eqref{loc.95}, \eqref{loc.97}, \eqref{loc.99}, \eqref{loc.101}, \eqref{loc.109}, \eqref{loc.111}, \eqref{loc.113}.
\begin{empheq}[box=\mymath]{gather}
\label{loc.115}
(\pa_r\phi)^2+(\pa_r\chi)^2+\pa_r^2f=0\\ \nonum \\
\scriptstyle{(\pa_v\phi)^2+(\pa_v\chi)^2+\pa_v^2f+\left(1-\frac{2m}{r}\right)(\pa_r\phi\pa_v\phi+\pa_r\chi\pa_v\chi+\pa_r\pa_vf)+\pa_r\left(\frac{m}{r}\right)\pa_vf}\nonum\\
\label{loc.116}
\hspace{2em}\scriptstyle{-\pa_v\left(\frac{m}{r}\right)\pa_rf+e^{2A}\pa_y\left(\frac{m}{r}\right)\pa_yf=f\left[\frac{2}{r^2}\pa_vm-\frac{e^{2A}}{r}(\pa_y^2m+4A'\pa_ym)\right]}\\ \nonum\\
\label{loc.117}
\pa_y\phi\pa_v\phi+\pa_y\chi\pa_v\chi+\pa_y\pa_vf-A'\pa_vf-\frac{\pa_ym}{r}\pa_rf=\frac{f}{r}\left(\frac{\pa_ym}{r}+\pa_r\pa_ym\right)\\ \nonum\\
\label{loc.118}
\pa_r\phi\pa_y\phi+\pa_r\chi\pa_y\chi+\pa_r\pa_yf-A'\pa_rf=0\\ \nonum\\
\label{loc.119}
\scriptstyle{r(\pa_r\phi\pa_v\phi+\pa_r\chi\pa_v\chi+\pa_r\pa_vf)-\pa_vf-\pa_rf\left(\pa_rm+1-\frac{3m}{r}\right)=f\left(\pa_r^2m-\frac{2}{r}\pa_rm\right)}\\ \nonum\\
\label{loc.120}
\scriptstyle{e^{-2A}\left[\pa_r\phi\pa_v\phi+\pa_r\chi\pa_v\chi+\pa_r\pa_vf-\pa_r\left(\frac{m}{r}\right)\pa_rf\right]+A'\pa_yf-(\pa_y\phi)^2-(\pa_y\chi)^2-\pa_y^2f=f\left(3A''+\frac{e^{-2A}}{r}\pa_r^2m\right)}\\ \nonum\\
\label{loc.121}
\scriptstyle{\frac{e^{-2A}}{r}\left[\pa_vf+\left(1-\frac{2m}{r}\right)\pa_rf\right]+A'\pa_yf-(\pa_y\phi)^2-(\pa_y\chi)^2-\pa_y^2f=f\left(3A''+\frac{2e^{-2A}}{r^2}\pa_rm\right)}
\end{empheq}

\newpage
\par Alternatively, the field equations in their extended form are given by equations \eqref{loc.96}, \eqref{loc.98}, \eqref{loc.100}, \eqref{loc.102}, \eqref{loc.110}, \eqref{loc.112}, \eqref{loc.114}.
\begin{empheq}[box=\mymath]{gather}
\label{loc.122}
(1+\pa_\phi^2f)(\pa_r\phi)^2+(1+\pa_\chi^2f)(\pa_r\chi)^2+2\pa_\chi\pa_\phi f\pa_r\chi\pa_r\phi+\pa_\phi f\pa_r^2\phi+\pa_\chi f\pa_r^2\chi=0\\ \nonum\\
\label{loc.123}
\begin{array}{l}
\scriptstyle{e^{-2A}}\left\{\scriptstyle{(1+\pa_\phi^2f)(\pa_v\phi)^2+(1+\pa_\chi^2f)(\pa_v\chi)^2+2\pa_\chi\pa_\phi f\pa_v\phi\pa_v\chi+\pa_\phi f\pa_v^2\phi+\pa_\chi f\pa_v^2\chi+\left(1-\frac{2m}{r}\right)[(1+\pa_\phi^2f)\pa_r\phi\pa_v\phi} \right.\\
\hspace{1.5em}\scriptstyle{+(1+\pa_\chi^2f)\pa_r\chi\pa_v\chi+\pa_\phi\pa_\chi f(\pa_r\phi\pa_v\chi+\pa_r\chi\pa_v\phi)+\pa_\phi f\pa_r\pa_v\phi+\pa_\chi f\pa_r\pa_v\chi]+\left(\frac{\pa_rm}{r}-\frac{m}{r^2}\right)(\pa_\phi f\pa_v\phi+\pa_\chi f\pa_v\chi)}\\
\hspace{1.4em}\left.\scriptstyle{-\frac{\pa_vm}{r}(\pa_\phi f\pa_r\phi+\pa_\chi f\pa_r\chi)+e^{2A}\frac{\pa_ym}{r}(\pa_\phi f\pa_y\phi+\pa_\chi f\pa_y\chi)}\right\}\scriptstyle{=f\left[\frac{2}{r^2}\pa_vm-\frac{e^{2A}}{r}(\pa_y^2m+4A'\pa_ym)\right]}
\end{array}\\ \nonum\\
\scriptstyle{(1+\pa_\phi^2f)\pa_y\phi\pa_v\phi+(1+\pa_\chi^2f)\pa_y\chi\pa_v\chi+\pa_\chi\pa_\phi f(\pa_y\chi\pa_v\phi+\pa_y\phi\pa_v\chi)+\pa_\phi f\pa_y\pa_v\phi}\nonum\\
\label{loc.124}
\scriptstyle{+\pa_\chi f\pa_y\pa_v\chi-A'(\pa_\phi f\pa_v\phi+\pa_\chi f\pa_v\chi)-\frac{\pa_ym}{r}(\pa_\phi f\pa_r\phi+\pa_\chi f\pa_r\chi)=\frac{f}{r}\left(\frac{\pa_ym}{r}+\pa_r\pa_ym\right)}\\ \nonum\\
(1+\pa_\phi^2f)\pa_r\phi\pa_y\phi+(1+\pa_\chi^2f)\pa_r\chi\pa_y\chi+\pa_\phi\pa_\chi f(\pa_r\chi\pa_y\phi+\pa_r\phi\pa_y\chi)\nonum\\
\label{loc.125}
+\pa_\phi f\pa_r\pa_y\phi+\pa_\chi f\pa_r\pa_y\chi-A'(\pa_\phi f\pa_r\phi+\pa_\chi f\pa_r\chi)=0\\ \nonum\\
\label{loc.126}
\begin{split}
&\scriptstyle{r[(1+\pa_\phi^2f)\pa_r\phi\pa_v\phi+(1+\pa_\chi^2f)\pa_r\chi\pa_v\chi+\pa_\phi\pa_\chi f(\pa_r\chi\pa_v\phi+\pa_r\phi\pa_v\chi)+\pa_\phi f\pa_r\pa_v\phi+\pa_\chi f\pa_r\pa_v\chi]}\\
&\scriptstyle{-(\pa_\phi f\pa_v\phi+\pa_\chi f\pa_v\chi)-\left(\pa_rm+1-\frac{3m}{r}\right)(\pa_\phi f\pa_r\phi+\pa_\chi f\pa_r\chi)=f\left(\pa_r^2m-\frac{2}{r}\pa_rm\right)}
\end{split}\\ \nonum\\
\label{loc.127}
\begin{split}
&\scriptstyle{e^{-2A}[(1+\pa_\phi^2f)\pa_r\phi\pa_v\phi+(1+\pa_\chi^2f)\pa_r\chi\pa_v\chi+\pa_\phi\pa_\chi f(\pa_r\chi\pa_v\phi+\pa_r\phi\pa_v\chi)+\pa_\phi f\pa_r\pa_v\phi+\pa_\chi f\pa_r\pa_v\chi}\\
&\scriptstyle{-\pa_r\left(\frac{m}{r}\right)(\pa_\phi f\pa_r\phi+\pa_\chi f\pa_r\chi)]+A'(\pa_\phi f\pa_y\phi+\pa_\chi f\pa_y\chi)-(1+\pa_\phi^2f)(\pa_y\phi)^2-(1+\pa_\chi^2f)(\pa_y\chi)^2}\\
&\scriptstyle{-2\pa_\phi\pa_\chi f\pa_y\phi\pa_y\chi-\pa_\phi f\pa_y^2\phi-\pa_\chi f\pa_y^2\chi=f\left(3A''+\frac{e^{-2A}}{r}\pa_r^2m\right)}
\end{split}\\ \nonum\\
\scriptstyle{\frac{e^{-2A}}{r}\left[\pa_\phi f\pa_v\phi+\pa_\chi f\pa_v\chi+\left(1-\frac{2m}{r}\right)(\pa_\phi f\pa_r\phi+\pa_\chi f\pa_r\chi)\right]+A'(\pa_\phi f\pa_y\phi+\pa_\chi f\pa_y\chi)-(1+\pa_\phi^2f)(\pa_y\phi)^2}\nonum\\
\label{loc.128}
\scriptstyle{-(1+\pa_\chi^2f)(\pa_y\chi)^2-2\pa_\phi\pa_\chi f\pa_y\phi\pa_y\chi-\pa_\phi f\pa_y^2\phi-\pa_\chi f\pa_y^2\chi=f\left(3A''+\frac{e^{-2A}}{r}\pa_r^2m\right)}
\end{empheq}
